Efficient-vDiT: Efficient Video Diffusion Transformers With Attention Tile

Despite the promise of synthesizing high-fidelity videos, Diffusion Transformers (DiTs) with 3D full attention suffer from expensive inference due to the complexity of attention computation and numerous sampling steps. For example, the popular Open-Sora-Plan model consumes more than 9 minutes for generating a single video of 29 frames. This paper addresses the inefficiency issue from two aspects: 1) Prune the 3D full attention based on the redundancy within video data; We identify a prevalent tile-style repetitive pattern in the 3D attention maps for video data, and advocate a new family of sparse 3D attention that holds a linear complexity w.r.t. the number of video frames. 2) Shorten the sampling process by adopting existing multi-step consistency distillation; We split the entire sampling trajectory into several segments and perform consistency distillation within each one to activate few-step generation capacities. We further devise a three-stage training pipeline to conjoin the low-complexity attention and few-step generation capacities. Notably, with 0.1% pretraining data, we turn the Open-Sora-Plan-1.2 model into an efficient one that is 7.4x -7.8x faster for 29 and 93 frames 720p video generation with a marginal performance trade-off in VBench. In addition, we demonstrate that our approach is amenable to distributed inference, achieving an additional 3.91x speedup when running on 4 GPUs with sequence parallelism.

==> _s3_motivation.tex <==

\section{Observations}

In the introduction:
We find repeat pattern in DiT. Moreover, this repeat pattern preserves the structure over different data points. Thus, enabling an opportunity to do a fixed pattern during training time.


Bottleneck of 3D-DiT lies in two dimensions: (1) Attention, (2) diffusion step. Fortunately, we observe there are redundancy in both dimensions (Fig. 1), (Fig. 2). Thus, we develop
\subsection{Characteristics of Attention}

\textbf{High computational cost of self-attention:} 3D-DiT consists of self-attention and cross-attention modules. Experimental results indicate that as the video resolution and the number of frames increase, the sequence length also increases, leading to a quadratic growth in the runtime of the attention modules. When the sequence length reaches 70,000, the runtime of self-attention accounts for 91.4\% of the entire 3D-DiT module, significantly challenging the speed of video generation.

\textbf{Attention map is not data-dependent:} The attention map of 3D-DiT has a dimension of [\texttt{seq\_len}, \texttt{seq\_len}]. As observed in Figure \texttt{fig:attn\_map}, the attention map exhibits a block pattern. According to the encoding rules of 3D-VAE, each block represents the information within a single frame of an image, while the blocks between them represent temporal information.

From Figure \texttt{fig:attn\_map}, for different prompt inputs, when fixing the layer and head, we observe that the pattern of the attention map remains the same for different input data, for both original model and consistent model (CM). Therefore, we conclude that the attention map is not data-dependent.

\subsection{Diffusion Step Redundancy}

\textbf{Redundancy between adjacent diffusion steps:} There exists a significant amount of similarity between adjacent diffusion steps. This redundancy can be eliminated through the distillation process of the consistent model.

\hangliang {@runlong Added more details.}
